Unconstrained Iris Segmentation using Convolutional Neural Networks

The extraction of consistent and identifiable features from an image of the human iris is known as iris recognition. Identifying which pixels belong to the iris, known as segmentation, is the first stage of iris recognition. Errors in segmentation propagate to later stages. Current segmentation approaches are tuned to specific environments. We propose using a convolution neural network for iris segmentation. Our algorithm is accurate when trained in a single environment and tested in multiple environments. Our network builds on the Mask R-CNN framework (He et al., ICCV 2017). Our approach segments faster than previous approaches including the Mask R-CNN network. Our network is accurate when trained on a single environment and tested with a different sensors (either visible light or near-infrared). Its accuracy degrades when trained with a visible light sensor and tested with a near-infrared sensor (and vice versa). A small amount of retraining of the visible light model (using a few samples from a near-infrared dataset) yields a tuned network accurate in both settings. For training and testing, this work uses the Casia v4 Interval, Notre Dame 0405, Ubiris v2, and IITD datasets.

==> coverpage.tex <==
{\Large \textbf{IPDPS Review Cover Letter}}
\\
\\
We thank the reviewers for their comments. The rebuttal below shows the improvements and betterments done after the review process.
\\

Reviewer 1
\\
\\
1.	Detailed explanation on the architecture is now provided in Section 4-B. In summary, the pragma set and unset is propagated to the cache controller via the core pipeline as an instruction. In the core it takes a single cycle, where it sets/unsets a special register. Once the register is set, marked store accesses are done via the L2 write partition. The “mark” is stored in the register, from where it is propagated to the cache controllers within cache message requests. From here, it is handled like any other request. All other accesses are done normally.
\\
2.	The proposed technique is compared with another prior work known as WCP utilizing cache partitioning to improve access latency in NVRAMs (comparison in Section 6-A,B). The compared work implements a hardware-only scheme that utilizes partitioning, moving lines to partitions that have high write locality. Our work is shown to outperform this prior work because only specific structures have unpredictable temporal write locality in machine learning and graph workloads, which our work can distinguish in software via pragmas.
\\

Reviewer 2
\\
\\
1.	Grammatical errors have been fixed.\\
2.	See Reviewer 1, Point 1.\\
3.	Cache memory models are known to be highly accurate in various simulators, hence the acquired performance improvements are expected to translate to real systems.\\

Reviewer 3
\\
\\
1.	Software tagging is utilized in various systems (such as Intel’s cache allocation technology that takes in software hints to optimize memory access latency). Our work uses it as a tool in a hardware-software combined approach to improve performance in NVRAM based machine learning and graph analytics.
\\
2.	A sensitivity study has been shown in the Section 6-E regarding variations in write latency (e.g. 2x or 5x slower write latency). Our work still shows improvements with these settings.
\\
3.	DRAM caches can be seen as analogous to LLCs. Hence adding a DRAM cache only mitigates the capacity problem, not the write access latency problem specifically.
\\

Review Synthesis.
\\
\\
1.	See Reviewer 1, Point 1.\\
2.	See Reviewer 1, Point 2.\\
3.	Typos and grammatical errors have been fixed in various sections.\\

Reviewer 4
\\
\\
1.	Advantages on having NVRAMs have been explained in Section 1 of the paper.\\
2.	The memory controller queue has a buffer size of 64 entries. Under general condition workloads, the queue size is not a problem. However, under the utilized machine learning and graph workloads, the queue is full more than 15\% of the total time on average across all workloads, which happens due to temporally changing write locality. This occurs due to thread access variations for each of the 256 threads, and variations across machine learning functions, and input graph characteristics. A study has been added to Section 6-D of the paper that shows improvements in NVRAM queue contention delays for various benchmarks in this regard\\
3.	LLC MPKI results are now shown and explained in Figure 4 and Section 4-C in the paper. The trend is similar to the LLC miss rate.\\

Reviewer 5
\\
\\
1.	Existing hardware-only partitioning approaches do not distinguish high distance write locality, and also have to cater for read locality. A comparative work utilizing such a partitioning scheme for NVRAMs (known as WCP) has been compared, and our scheme improves 10\% over it in performance.\\
2.	Conventional multicores such as Xeon Phi have several MB in LLC cache capacities. This work has an LLC capacity of 16MB, which is in sync with current multicore trends.\\
3.	See Reviewer 4, Point 3.\\

